LMStream: When Distributed Micro-Batch Stream Processing Systems Meet GPU

This paper presents LMStream, which ensures bounded latency while maximizing the throughput on the GPU-enabled micro-batch streaming systems. The main ideas behind LMStream's design can be summarized as two novel mechanisms: (1) dynamic batching and (2) dynamic operation-level query planning. By controlling the micro-batch size, LMStream significantly reduces the latency of individual dataset because it does not perform unconditional buffering only for improving GPU utilization. LMStream bounds the latency to an optimal value according to the characteristics of the window operation used in the streaming application. Dynamic mapping between a query to an execution device based on the data size and dynamic device preference improves both the throughput and latency as much as possible. In addition, LMStream proposes a low-overhead online cost model parameter optimization method without interrupting the real-time stream processing. We implemented LMStream on Apache Spark, which supports micro-batch stream processing. Compared to the previous throughput-oriented method, LMStream showed an average latency improvement up to a maximum of 70.7%, while improving average throughput up to 1.74x.

==> _Deprecated_Abstract.tex <==
\label{sec:abstract}%실시간으로 인입되는 데이터에 온라인 분석을 수행하는 stream processing에 대한 수요가 증가하고 있다. 데이터 인입 속도가 점점 빨라지고, 그 양이 폭발적으로 증가하는 만큼 stream systems에서도 GPU를 이용하여 처리 속도를 증가시키고자 하는 시도가 계속되고 있다. GPU를 fully utilizing 하려면 일반적으로 일정 수준 이상의 데이터가 처리되어야 한다. 따라서 stream processing에서 GPU를 사용할 경우에도 real-time data를 일정 기간동안 모아서 한번에 처리하는 방법이 다수 사용된다. 이러한 방식은 throughput을 향상시키는데 도움이 되지만, 실시간으로 인입되는 stream data의 개별적인 latency는 크게 손상된다. Throughput-oriented 시스템의 또 다른 특징은 모든 operator들을 GPU로 offloading한다는 것이다. 이는 서로 다른 device간 데이터 통신 오버헤드를 피하기 위함이다. 그러나 이 경우 device preference에 따라 query operator를 더욱 fine-grained하게 분배하여 얻을 수 있는 최적화 기회를 놓치게 된다. 이러한 device preference는 처리하는 데이터의 크기에 따라 변화하므로, 다양한 크기의 데이터가 연속적으로 인입되는 스트리밍 환경에서는 이를 반영하는 것이 중요하다. 본 논문에서 제시하는 CG-Spark는 이러한 문제를 해결하기 위해 stream processing system에서 개별 데이터마다 일정 수준 이하의 latency를 유지하면서 GPU를 사용할 수 있도록 한다. 이 때 operator마다 서로 다른 device preference(CPU or GPU)를 가진다는 점을 이용하여, query 내 operator를 적절한 device에 mapping하여 throughput이 optimize될 수 있도록 한다. 또한 실시간으로 인입되는 data traffic과 전체 시스템 성능을 모니터링하여, 적절한 크기의 micro-batch를 구성하고 그에 따른 operator 별 dynamic device mapping 을 통해 최적화된 execution plan을 만든다. CG-Spark는 latency와 throughput을 동시에 개선하려는 목적을 달성하기 위해 cost models와 rules를 사용하여 query 실행 계획을 설립한다. 이 과정에서 사용자가 명시한 deadline time이나 가용 GPU memory 크기가 실시간으로 반영되어 사용자의 요구사항이 만족되고 시스템이 안정적으로 운영될 수 있도록 한다. \texttt{CG-Spark}는 micro-batch 방식의 stream processing을 지원하는 Spark에서 구현되었다. 모든 operator를 GPU로 offloading하는 original Spark와 비교하여, \texttt{CG-Spark}의 throughput은 약 \textcolor{blue}{?%} 향상되었다. 또한 trigger를 이용해 static buffering을 진행하는 방식과 비교하여, \texttt{CG-Spark}의 tail latency는 약 \textcolor{blue}{?%} 향상되었다.
Recently, the demand for stream processing systems that perform online analysis on real-time data is increasing. As the data ingestion speed is getting faster and the amount of data is also increasing, there have been various attempts to accelerate the processing speed of streaming systems by using the GPU. 
%To fully utilize the GPU, data above a certain level needs to be processed. Therefore, for GPU utilization in stream processing, many previous studies collect real-time data for a constant time and process it at once. 
Many previous studies collect real-time data for a constant time period and process it at once to fully utilize the GPU.
Although this method improves the overall throughput, the individual latency of the real-time stream data is considerably damaged.
%
Another characteristic of throughput-oriented systems is that they offload all operators to the GPU to avoid data communication overhead between different devices. However, in this case, systems lose optimization opportunities obtained by distributing the query operator more fine-grained way according to device preference. Specifically, these device preferences change depending on the size of the data. Therefore, it is necessary to reflect dynamic device preferences in streaming environments where data of varying sizes are continuously collected.
%
In this paper, we present \texttt{CG-Spark}, a new stream processing system, which maximizes the throughput by using the GPU, while keeping the latency of each data below a certain level simultaneously. 
%
%At this point, taking advantage of the fact that each query operator has a different device preference (CPU or GPU), systems can optimize throughput by mapping the operator to the appropriate device. \texttt{CG-Spark} achieves the goal of improving both latency and throughput by using specific cost models and rules. If there is a user-specified deadline time, \texttt{CG-Spark} uses deadline-aware cost models so that the latency of each data does not violate the deadline. In addition, stability is essential in a stream processing system that continuously processes data at high speed. For system stability, CG-Spark monitors the available GPU memory size in real-time, and the value is reflected in the cost model. Therefore, \texttt{CG-Spark} prevents system failure due to insufficient GPU memory.
%
First, \texttt{CG-Spark} construct a micro-batch of an appropriate size by monitoring real-time input data traffic and overall systems performance. Then, \texttt{CG-Spark} create an optimized execution plan for every micro-batch through dynamic device mapping per each operator. \texttt{CG-Spark} establishes a query execution plan using cost models and rules to achieve the goal of simultaneously improving latency and throughput. They reflect the deadline time specified by the user and the size of the available GPU memory capacity. This allows \texttt{CG-Spark} to satisfy the user's requirements and operate the streaming process stably.
%
We implement \texttt{CG-Spark} on Apache Spark that supports micro-batch type stream processing. Compared to the original Spark, which offloads all operators to the GPU, the throughput of \texttt{CG-Spark} is improved by about \textcolor{blue}{?\%}. Also, compared to the method of static buffering using the trigger, the tail latency of \texttt{CG-Spark} is improved by about \textcolor{blue}{?\%}.

==> _Deprecated_Evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

\subsection{Experimental Setup}\label{subsec:experimentalSetup}

\textcolor{blue}{%본 논문에서 제시한 시스템의 효율성을 보이고자, original Spark에 다양한 시스템을 구현하여 성능 비교를 진행하였다. (\textbf{OS(t$N$)})은 throughput-oriented 방식을 벤치마크 하기 위한 시스템으로, trigger를 사용해 $N$초 동안 buffering을 진행하고 한번에 GPU로 보내 처리한다. (\textbf{OSCP(t$N$)})은 (\textbf{OS(t$N$)})의 시스템에 constant device preference 방식을 추가한 경우이다. \texttt{LMStream}의 경우, deadline이 없는 (\textbf{CG(d0)})와, deadline이 $N$초인  (\textbf{CG(d$N$)})으로 나누었다.
To show the \texttt{LMStream}'s efficiency presented in this paper, we simulated various target systems using the original Spark and compared their performance. \textbf{OS(t$N$)} is a system for evaluating the throughput-oriented method, which uses a trigger to buffer data for $N$ seconds and sends it to the GPU for processing. \textbf{OSCP(t$N$)} is a system where the constant device preference method is applied to the \textbf{OS(t$N$)}. In the case of \texttt{LMStream}, we use two systems such as \textbf{CG(d0)} with no deadline and \textbf{CG(d$N$)} with a deadline of $N$ seconds.}

% IPDPS에서는 사용하지 않음
\begin{comment}
%%%%%%%%%%%%%%% [Evaluation - Experimental Setup] Table 2: experimentalSetup %%%%%%%%%%%%%%%%
\setlength{\extrarowheight}{2pt}
\begin{table}[H]
    \centering
    %\captionsetup{labelfont={color=red},font={color=red}}
    \caption{Real-world streaming workloads used in our experiments. Each query details are presented in ~\cite{Saber}.}
    \vspace{-0.07in}
    \color{blue}
    \begin{tabular}{|c|c|c|c|}
        \hline%\hline
        \strut
        \textbf{Benchmark} & \textbf{Data Size} & \textbf{Query Type~\cite{Saber}} & \textbf{Notation} \\
        \hline%\hline
        \multirow{2}{*}{\makecell{Linear \\ Road~\cite{Linear-Road-Bench}}}
            & \multirow{2}{*}{\makecell{70 B \\ (per record, fixed)}}
            & \multirow{1}{*}{Query 3} & LR1 \\
            \cline{3-4}
            &  & \multirow{1}{*}{Query 4} & LR2 \\
        \specialrule{.14em}{.1em}{.1em}
        \multirow{2}{*}{\makecell{Cluster \\ Monitoring~\cite{Google-Cluster-Monitoring-Bench}}}
            & \multirow{2}{*}{\makecell{130 $\sim$ 145 B \\ (per record, variable)}}
            & \multirow{1}{*}{Query 1} & CM1 \\
            \cline{3-4}
            &  & \multirow{1}{*}{Query 2} & CM2 \\ \hline
        %\specialrule{.14em}{.1em}{.1em}
        %\makecell{Synthetic \\ Stream + Batch} & \makecell{60 B stream record \\ 1.7 GB batched file} & Query 2 of LR & SSB \\
            %\hline%\hline
    \end{tabular}
    %\vspace{-0.15in}
\label{tab:experimentalSetup}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

% 논문에서의 위치 상 문제로 여기에 우선 배치함
%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageProcessThroughput.pdf}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{Average throughput during entire query for each workload. Our definition of average throughput follows  Equation~\ref{eq:averageThroughput}.}}
    \vspace{-0.2in}
\label{fig:avgProcessThroughput}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageLatency.pdf}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{Average latency during entire query for each workload. Our definition of average latency follows  Equation~\ref{eq:averageLatency}.}}
    \vspace{-0.2in}
\label{fig:avgLatency}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.1cm}
\noindent{\textbf{Configurations.}}\label{subsubsec:expConfigurations} \textcolor{blue}{%실험을 위해 1대의 master 노드와 2대의 worker 노드로 이루어진 Spark 클러스터를 구성하였다. 각 worker 노드에는 두 개의 executor가 실행되며, 각 executor마다 CPU 코어 12개, host 메모리 24G, GPU 1개, device memory 8G 씩을 할당하여 사용하였다. CPU는 Intel Xeon Silver 4210 모델을 사용하였으며, GPU는 NVIDIA GeForce RTX 2080 Ti 모델을 사용하였다.
For the experiment, we configured a Spark cluster consisting of one master node and two worker nodes. We placed two executors per worker node. Each executor uses 12 CPU cores, 24 GB host memory, 1 GPU, and 8 GB device memory as resources. The types of CPU and GPU are the Intel Xeon Silver 4210, and the NVIDIA GeForce RTX 2080 Ti, respectively.}

\vspace{0.1cm}
\noindent{\textbf{Workloads and Stream Traffic Types.}}\label{subsubsec:expWorkloads} \textcolor{blue}{%실험에 사용한 워크로드와 구성은 Table~\ref{tab:experimentalSetup}에 정리하였다. LR benchmark와 CM benchmark는 real-world streaming benchmark으로 filter, project, aggregate, join 등을 포함한 다양한 query operation을 수행한다. 실험에 사용한 data traffic은 아래와 같은 세 가지 종류를 사용하였다.
The workloads used in the experiments are summarized in Table~\ref{tab:experimentalSetup}. The Linear Road benchmark~\cite{Linear-Road-Bench} and Cluster Monitoring benchmark~\cite{Google-Cluster-Monitoring-Bench} are real-world streaming benchmarks that perform various query operations, including filter, project, aggregate, and join. We used the following three types of data traffic in our experiments.
\begin{itemize}
    \item Basic [\textbf{B($N$)}]: Generates a constant number of ($N$*1000) records every second.
    \item Uniform [\textbf{U($N$)}]: Generates a random record that converges to a specific average value ($N$*1000) every second.
    \item Random [\textbf{R($L$, $U$)}]: Generates a random record with a lower limit value ($L$*1000) and an upper limit value ($U$*1000) every second.
\end{itemize}}

\begin{comment} % 논문 상의 위치를 위해 design.tex로 옮김
%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageProcessThroughput.pdf}
    \vspace{-0.2in}
    \caption{Average throughput during entire query for each workload. Our definition of average throughput follows Equation~\ref{eq:averageThroughput}.}
    \vspace{-0.2in}
\label{fig:avgProcessThroughput}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageLatency.pdf}
    \vspace{-0.2in}
    \caption{Average latency during entire query for each workload. Our definition of average latency follows  Equation~\ref{eq:averageLatency}.}
    \vspace{-0.1in}
\label{fig:avgLatency}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

\subsection{Overall Performance}\label{subsec:overallPerformance}

\begin{comment}
%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageProcessThroughput.pdf}
    \vspace{-0.2in}
    \caption{Average throughput during entire query for each workload. Our definition of average throughput follows  Equation~\ref{eq:averageThroughput}.}
    \vspace{-0.2in}
\label{fig:avgProcessThroughput}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% [Evaluations - averageProcessThroughput] %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/averageLatency.pdf}
    \vspace{-0.2in}
    \caption{Average latency during entire query for each workload. Our definition of average latency follows  Equation~\ref{eq:averageLatency}.}
    \vspace{-0.1in}
\label{fig:avgLatency}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

% 논문에서 그림의 위치 상 여기에 먼저 배치함
%%%%%%%%%%%%%%%%% [Evaluations - timelineLatency] %%%%%%%%%%%%%%%%%
\begin{figure*}
    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/timeline_latency_and_size.pdf}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{The uppermost bold line is the tail latency per micro-batch. The definition of average latency follows Equation~\ref{eq:tailLatency}. Since the traffic is B(1), a wider latency range indicates more individual datasets per micro-batch.}}
    \vspace{-0.2in}
\label{fig:timelineLatencyAndSize}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{%이번 section에서는 다른 기존의 mechanism과 \texttt{LMStream}의 기본적인 성능 비교를 진행한다. 각 워크로드를 30분동안 실행시킨 뒤 매 micro-batch마다 발생한 throughput과 latency값의 평균을 계산하였으며, 각 metric은 Section~\ref{subsec:problemDefinition}에서 정의한 equation~\ref{eq:averageThroughput}, \ref{eq:averageLatency}에 따라 측정하였다.
This section compares the primary performance of \texttt{LMStream} with those of other existing mechanisms. After running each workload for 30 minutes, we measured the average throughput and latency during entire query. Each metric is measured according to Equation~\ref{eq:averageThroughput}, \ref{eq:averageLatency} in Section~\ref{subsec:problemDefinition}.}

\textcolor{blue}{%Figure~\ref{fig:avgProcessThroughput}에서는 시스템마다의 average throughput을 보여준다. 일정 기간 무조건적인 buffering을 진행하는 OS(t3)에 비해, \texttt{LMStream}의 average throughput은 거의 동일하게 유지되거나 더 높은 값을 가진다. Deadline이 0인 CG(d0)의 경우, as-soon-as-possible policy를 이용하여 latency가 우선시된다. 그러나 operator마다 dynamic device preference를 반영하므로 무조건적으로 GPU를 사용하는 OS(t3)보다 throughput이 최적화된다. 특히 작은 데이터가 비교적 많이 인입되는 B(1)이나 U(2.5)의 경우, 오히려 OS(t3)보다 average throughput이 높게 나타나기도 한다. 반면 데이터 크기가 큰 B(2.5)의 경우 결과적으로는 모든 operator가 GPU를 사용하도록 설정될 것이다. 따라서 OS(t3)보다 planning 과정에서 발생하는 오버헤드만 추가될 뿐이므로 average throughput이 낮아질 수 있다. 전반적으로 throughput 값은 OS(t3)와 비슷하게 유지된다. Deadline이 5인 CG(d5)의 경우, deadline을 준수하는 선에서 buffering을 유지한다. 따라서 OS(t3)보다 average throughput이 높은 경우가 대부분이다. OSCP(t0)의 경우, 데이터 크기와 관계없이 static device preference를 가진다. Section~\ref{subsec:ourObservations}에서 밝힌 바와 같이, 데이터의 크기가 커지면 모든 operator가 GPU를 선호하게 된다. 따라서 이러한 점을 고려하지 않은 경우이므로 average throughput이 가장 낮다. 특히 데이터의 크기가 큰 B(2.5)의 경우에도 기존의 CPU preference가 유지되기 때문에, 처리 성능이 악화된다.
Figure~\ref{fig:avgProcessThroughput} shows the average throughput of each system. In the case of CG(d0) with a deadline of 0, \texttt{LMStream} prioritizes latency using the as-soon-as-possible policy. Nevertheless, since it reflects dynamic device preference for each operator, throughput is optimized compared to OS(t3) that unconditionally uses GPU. In particular, when the traffic is B(1) or U(2.5), which generates relatively large amounts of small data, the average throughput is rather higher than that of OS(t3). On the other hand, when the traffic is B(2.5), which constantly generates relatively large data, all operators will eventually use the GPU. Therefore, the throughput is compromised compared to OS(t3) because \texttt{LMStream}'s planning overhead becomes dominant in processing. Overall, the throughput value is higher or similar to OS(t3). In the case of CG(d5) with a deadline of 5, buffering period is maintained at the line that meets the deadline. Therefore, its average throughput is the highest, up to 2.1$\times$ higher than OS(t3). OSCP(t0) has static device preference regardless of data size. As stated in Section~\ref{subsec:ourObservations}, all operators prefer GPU as data size increases. OSCP(t0) does not reflect the dynamic device preference and shows the lowest average throughput. Specifically, if the traffic is B(2.5) or U(2.5), OSCP(t0) sets some operators to run on the CPU regardless of the size of the data, which significantly reduces processing performance.}

\textcolor{blue}{%Figure~\ref{fig:avgLatency}에서는 시스템마다의 average latency를 보여준다. 모든 결과에서 CG(d0)는 확연히 낮은 latency를 보여준다. CG(d5)는 as-late-as-policy에 따라 모든 micro-batch가 설정된 deadline인 5초 내외로만 처리되도록 한다. 따라서 비교적 높은 average latency를 보이지만, 그 값은 5초 내로 수렴한다. LR2의 경우에는 CG(d5)의 average latency 값이 5초보다 조금 높게 나타난다. 이것은 LR2의 계산량이 많아 deadline 준수와 throughput 유지를 동시에 달성하기 힘들기 때문이다. 이에 대해서는 이후 section~\ref{subsec:deadlineViolationRate}에서 더 자세히 다룬다. OS(t3)은 매번 3초 동안 일정하게 buffering을 수행하므로 모든 micro-batch가 3초 이상의 latency를 가지게 되며, 이는 매우 비효율적이다. OSCP(t0)는 buffering은 하지 않으나, static device preference로 인해 성능이 저하되고, 길어지는 processing time으로 인해 높은 latency가 발생하게 된다.
Figure~\ref{fig:avgLatency} shows the average latency of each system. In all results, CG(d0) shows significantly lower average latency. Its latency is improved up to a maximum of 25.8\% compared to OS(t3). CG(d5) allows all micro-batches to be processed only within 5 seconds according to the as-late-as-policy. Therefore, it shows relatively high average latency, but the value converges within 5 seconds. In LR2, the average latency value of CG(d5) is slightly higher than 5 seconds.  This indicates that achieving deadline compliance and throughput maintenance at the same time is difficult due to the large amount of computation in LR2. We will deal with this issue in more detail later in Section~\ref{subsec:deadlineViolationRate}. OS(t3) performs buffering for 3 seconds each time. Every micro-batch has a latency of 3 seconds or more, which is very inefficient. OSCP(t0) does not buffer, but its static device preference degrades the overall performance. Longer processing time leads to the highest latency value among all.}

\subsection{Changes in Tail Latency and Data Size Over Time}\label{subsec:timelineOfTailLatencyAndDataSize}

%%%%%%%%%%%%%%%%% [Evaluations - timelineThroughput] %%%%%%%%%%%%%%%%%
%\begin{figure*}[t]
%    \centering\includegraphics[width=\textwidth,keepaspectratio]{figures/timeline_throughput.pdf}
%    \vspace{-0.2in}
%    \caption{TMP}
%    \vspace{-0.2in}
%\label{fig:timelineThroughput}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{%이번 section에서는 micro-batch 내의 개별적인 dataset 별로 측정되는 tail latency 값과을 시간의 흐름에 따라 나타내었다. 해당 실험 결과에서 micro-batch마다 처리한 데이터 크기의 변화량도 함께 확인할 수 있다. Tail latency는 Section~\ref{subsec:problemDefinition}에서 정의한 equation~\ref{eq:tailLatency}에 따라 측정하였다. 가장 성능이 좋지 않은 OSCP(t0)는 실험에서 제외하였다. 결과 그래프는 대표적으로 LR1-B(1000)에 대해서만 나타내었다.
This section presents the changes in tail latency measured for individual dataset per micro-batch over time. We also show the variation in the processed data size per micro-batch. Tail latency metric was measured according to Equation~\ref{eq:tailLatency} defined in Section~\ref{subsec:problemDefinition}. We have excluded the least performing OSCP(t0) from the experiments from now on. Therefore, the resulting graph is shown only for LR1-B(1).}

\textcolor{blue}{%Figure~\ref{fig:timelineLatencyAndSize}를 보면 OS(t3)은 모든 micro-batch의 tail latency가 고정된 buffering time인 3초를 넘게 된다. 더 큰 문제는 tail latency 값이 시간이 지남에 따라 점점 더 증가한다는 것이다. LR1의 경우, query 계산량이 많아 큰 데이터를 한꺼번에 처리하는 데 걸리는 시간이 길다. 따라서 전반적인 시스템 상관없이 무조건적인 buffering을 지속하면, processing time이 길어짐에 따라 처리해야 할 데이터가 점점 더 커지는 악순환이 지속된다. 실제로 OS(t3)의 경우는 이후 tail latency가 계속 증가하여 deadline violation rate가 매우 크게 나타난다. 이 부분은 이후 section~\ref{subsec:deadlineViolationRate}에서 실험으로 보인다.
As shown in Figure~\ref{fig:timelineLatencyAndSize}, the tail latency of every micro-batch in OS(t3) exceeds the fixed buffering time of 3 seconds. To make matters worse, the tail latency increases over time. Note that it takes a long time to process large data at once in LR1 because of the large amount of query calculation. Suppose that the system starts to spend a long time for a processing phase. Since traffic continues to generate new data while processing for a more extended period, subsequent micro-batch must process more data. As a result, end-to-end latency continues to increase, falling into a faulty cycle. In fact, the tail latency continues to increase after that, resulting in a tremendous deadline violation rate. We will discuss this issue later in Section~\ref{subsec:deadlineViolationRate}.}

\textcolor{blue}{%반면 \texttt{LMStream}의 경우, 실시간 시스템 상황에 따라 단일 micro-batch에서 처리할 데이터의 크기를 변화시킨다. CG(d0)의 경우, average latency를 낮추기 위해 micro-batch 당 데이터의 크기를 점점 감소시키는 것을 확인할 수 있고, 그에 따라 tail latency도 점점 감소한다. 약 14분여부터는 tail latency가 다시 상승하게 되는데, 이는 시스템의 throughput이 너무 낮아지는 것을 방지하기 위해 시스템에서 자체적으로 target latency를 높이기 때문이다. CG(d5)의 경우, 5초로 bound 되는 선에서 최대의 tail latency 값을 유지하는 것을 확인할 수 있다. 따라서 처리하는 데이터의 양이 많이 throughput이 높게 나타난다. CG(d5)는 user-required deadline을 만족하는 것을 우선시한다. 따라서 워크로드에서 계산량이 많아지면 latency를 손상시키는 대신 한번에 처리하는 데이터의 양을 줄인다. Figure~\ref{fig:timelineLatencyAndSize}의 맨 오른쪽 그래프를 보면, 이와 같은 동작 방식으로 average latency를 꾸준하게 유지하는 것을 확인할 수 있다.
On the other hand, \texttt{LMStream} adaptively controls the size of data within a single micro-batch according to the real-time system situation. In CG(d0), the size of data per micro-batch is gradually reduced to lower tail latency, reducing average latency accordingly. After about 14 minutes, the tail latency rises again because the system raises the target tail latency to prevent the system's throughput from being too low. In CG(d5), the maximum tail latency value is maintained at the line bounded by 5 seconds. Buffering until just before the deadline allows \texttt{LMStream} to handle large amounts of data, which results in the highest throughput. Still, CG(d5) prioritizes satisfying the user-required deadline. Thus, when the amount of computation in the workload increases, \texttt{LMStream} reduces the amount of data processed at one time instead of compromising tail latency. In the graph on the far right of Figure~\ref{fig:timelineLatencyAndSize}, it is shown that CG(d5) sustains the average latency by reducing the micro-batch data size after about ten minutes.}

% GPU memory 부분은 제외
\begin{comment}
\subsection{GPU Device Memory Usage}\label{subsec:GPUDeviceMemoryUsage}

%%%%%%%%%%%%%%%%% [Evaluations - GpuDeviceMemoryUsage] %%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering\includegraphics[width=\linewidth,keepaspectratio]{figures/gpuMemOOM.pdf}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{GPU device memory usage per micro-batch. OS(t3) failed intermediately due to an out-of-memory error.}}
    %\vspace{-0.2in}
\label{fig:gpuOOM}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{%이번 section에서는 \texttt{LMStream}의 GPU out-of-memory 방지 효율성을 보인다. GPU 가용 메모리가 부족해진 상황을 시뮬레이션 하기 위해 device memory는 executor 당 1G씩만 할당하였고 traffic은 B(20)을 사용하였다. 실험 결과는 대표적으로 LR1에 대해서만 나타내었다.
This section shows the efficiency of \texttt{LMStream}'s mechanism for preventing GPU out-of-memory errors. For this, only 1 GB of device memory is allocated per executor to simulate the situation in which the available memory of the GPU is insufficient. We used B(20) as data traffic. Experimental results are shown only for LR1.}

\textcolor{blue}{%Figure~\ref{fig:gpuOOM}에서는 시간에 따른 GPU memory 사용량을 보인다. 실험 결과 OS(t3)의 경우, 어플리케이션 시작 후 약 1시간이 지나자 GPU 메모리가 부족해져 system fail이 발생하였다. 반면 \texttt{LMStream}에서는 GPU 메모리가 약 8000 MB 내외로 유지되면서 시스템이 정상 유지되었다. 이를 통해 \texttt{LMStream}의 GPU memory usage aware execution planning이 스트리밍 시스템의 요구 조건인 stability를 높인다는 것을 확인할 수 있다. 다만 주어진 device memory는 1 GB인데 비해, \texttt{LMStream}의 최대 device memory usage는 약 0.8 GB로 약간 부족한 편이다. 따라서 매 micro-batch 실행과는 분리된 조금 더 세밀한 resource management가 필요할 수 있다.
Figure~\ref{fig:gpuOOM} shows the GPU memory usage over time. In OS(t3), the GPU memory ran out, and a system failure occurred about an hour after the application started. On the other hand, \texttt{LMStream} kept the GPU memory at around 0.8 GB and worked normally without errors for the next few hours. This confirms that \texttt{LMStream}'s execution planning being aware of GPU memory usage increases stability, which is a crucial requirement of streaming systems. However, while the given GPU memory is 1 GB, the maximum device memory usage of \texttt{LMStream} is about 0.8 GB, which is slightly less than the theoretical maximum. We conjecture that more granular resource management separate from every micro-batch run is needed to increase the maximum usage.}
\end{comment}

%%%%%%%%%%%%%%% [Evaluations - violationRate] %%%%%%%%%%%%%%%%

\setlength{\extrarowheight}{2pt}
\begin{table}[t]
    \color{blue}
    \centering
    %\captionsetup{justification=centering}
    \caption{Violation rate when deadline is 5 seconds.}
    \vspace{-0.07in}
    \centering
    \setlength\tabcolsep{3pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \textbf{Violation Rate} & \textbf{LR1-U(2.5)} & \textbf{LR1-R(0.1, 5)} & \textbf{CM1-U(2.5)} & \textbf{CM1-R(0.1, 5)} \\ \hline
        \textbf{OS(t3)} & 0.618 & 0.568 & 0.463 & 0.321 \\ \hline
        %\rowcolor{LightCyan}
        \textbf{CG(d5)} & 0.152 & 0.122 & 0.116 & 0.108 \\ \hline
    \end{tabular}
    \vspace{-0.1in}
\label{tab:violationRate5sec}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%% [Evaluations - violationRate] %%%%%%%%%%%%%%%%

\setlength{\extrarowheight}{2pt}
\begin{table}[t]
    \color{blue}
    \centering
    %\captionsetup{justification=centering}
    \caption{Violation rate when deadline is 7 seconds.}
    \vspace{-0.07in}
    \centering
    \setlength\tabcolsep{3pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \textbf{Violation Rate} & \textbf{LR1-U(2.5)} & \textbf{LR1-R(0.1, 5)} & \textbf{CM1-U(2.5)} & \textbf{CM1-R(0.1, 5)} \\ \hline
        \textbf{OS(t3)} & 0.418 & 0.329 & 0.31 & 0.243 \\ \hline
        %\rowcolor{LightCyan}
        \textbf{CG(d7)} & 0.109 & 0.076 & 0.069 & 0.035 \\ \hline
    \end{tabular}
    %\vspace{-0.1in}
\label{tab:violationRate7sec}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% [Evaluations - violationRate] %%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering\includegraphics[width=\linewidth,keepaspectratio]{figures/violationRate_withoutTotal_modified.pdf}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{The number of datasets per micro-batch which violated the user-required deadline.}}
    %\vspace{-0.2in}
\label{fig:numViolationPerBatch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Deadline Violation Rate}\label{subsec:deadlineViolationRate}

\textcolor{blue}{%이번 section에서는 본 시스템의 추가적인 feature인 deadline이 실제로 만족되는지에 대해 다룬다. Realistic 환경을 위해 fluctuating traffic을 사용하였고, 각 워크로드마다 1시간 씩 실험을 진행하였다. 결과는 LR1에 대해서만 나타내었다. Table~\ref{tab:violationRate5sec}과 Table~\ref{tab:violationRate7sec}에서는 fluctuating traffic에서 deadline이 각각 5초, 7초일 때 violation rate(\#violation / \#total)을 나타낸다. 실험 결과 모든 경우에서 OS(t3)보다 \texttt{LMStream}의 deadline violation rate가 훨씬 낮았다. 특히 static buffering을 진행하는 경우, 워크로드에 따라 tail latency가 지속적으로 증가하는 경향을 보이기 때문에 시간이 갈 수록 violation rate가 증가한다. Figure~\ref{fig:numViolationPerBatch}는 LR1에서 매 micro-batch마다 deadline violation이 발생한 dataset의 개수를 나타낸 그래프이다. Figure~\ref{fig:numViolationPerBatch}의 왼쪽 그래프를 보면 시간이 지날수록 OS(t3)의 violation dataset 개수가 점점 증가하는 것을 볼 수 있다. 반면 CG(d5)의 violation dataset의 개수는 1개 내로 일정하게 유지된다.
This section discusses the deadline violation rates of each system. We used fluctuating traffics to simulate a realistic environment and conducted experiments for about 90 minutes for each workload. Due to the lack of space, results are shown only for LR1. Table~\ref{tab:violationRate5sec} and Table~\ref{tab:violationRate7sec} show the violation rate (\#violation / \#total) when the deadlines are 5 and 7 seconds, respectively. The deadline violation rate of \texttt{LMStream} was much lower (i.e., improved up to a maximum of 78.5\%) than that of OS(t3) in all cases. In particular, static buffering method causes violation rate to increase as time goes by. This is because tail latency tends to increase continuously depending on the workload. Figure~\ref{fig:numViolationPerBatch} shows the number of datasets in which deadline violation occurred for every micro-batch. In Figure~\ref{fig:numViolationPerBatch}, the number of violation datasets in OS(t3) gradually increases as time goes by. On the other hand, the number of violation datasets in CG(d5) is kept constant within one.}

\textcolor{blue}{%한편 \texttt{LMStream}에서 약간의 deadline violation이 발생하는 이유는 \texttt{LMStream}가 stream processing system의 throughput도 어느 정도 유지하기 때문이다. 즉, \texttt{LMStream}는 hard deadline 정책을 따르기 보다는 시스템의 전반적인 성능을 복합적으로 고려한다. 만약 \texttt{LMStream}에서 일정 수준의 violation이 계속해서 발생한다면, deadline 준수와 throughput 유지를 동시에 수행하기에는 실질적인 processing capacity가 부족한 것으로 판단할 수 있다. 실제로 deadline을 7초로 늘려 실험한 Table~\ref{tab:violationRate7sec}의 경우를 보면, violation rate가 훨씬 더 감소하여 0에 수렴함을 확인할 수 있다.
The reason for some deadline violations in \texttt{LMStream} is because \texttt{LMStream} also maintains the throughput of the stream processing system to some extent.
%In other words, \texttt{LMStream} considers the overall performance of the system in a complex way. %밑 문장에서도 어차피 설명하므로 아예 삭제하였습니다.
%rather than following the hard deadline policy.
If a certain percentage of violations continue to occur in \texttt{LMStream}, one possibility is that the actual processing capacity is insufficient to maintain throughput while meeting the deadline. Indeed, increasing the deadline to sufficient values further reduces the violation rate. In Table~\ref{tab:violationRate7sec}, the deadline violation rate of CG(d7) converges to almost zero.}


%\subsection{Efficiency of optimization}\label{subsec:efficiencyOfOptimization}

%마지막으로 본 시스템의 target performance 값과 그에 따른 optimization의 적절성을 보인다. \textcolor{blue}{Figure~\ref{}}에서 시간대 별 target performance와 실제 performance 값을 비교하여 나타내었다. Traffic은 B(1000), B(10000), U(5000), R(1000, 10000)을 사용하였으며, deadline 옵션이 없는 C0와 deadline이 5초로 설정된 C5에 대해 모두 실험을 진행하였다.

%\subsection{Scalability}\label{subsec:scalability}

%Spark executor나 worker 늘려가면서 실험 가능

==> _Deprecated_Motivation.tex <==
\section{Motivation}\label{sec:motivation}

%본 장에서는 이전 연구들의 특징과 이로 인해 야기될 수 있는 문제점을 설명한다. 그리고 이를 해결하기 위해 사용한 본 논문의 핵심 접근법을 설명하고, 이의 타당성을 간단한 실험을 통해 제시한다.
In this section, we describe the characteristics of previous studies and the problems they cause in stream processing systems. Furthermore, we report several observations to motivate the main idea of \texttt{CG-Spark}'s design. 
%We present our approach's validity through a simple experiment.

\subsection{Previous Works}\label{subsec:previousWorks}

\noindent{\textbf{Throughput-oriented Approach.}}\label{subsubsec:throughputOrientedApproach}
%스트리밍 시스템에서 GPU를 도입한 다른 연구들은 공통적으로 throughput에 중점을 두었다. 따라서 GPU를 fully utilize 하기 위해 data를 buffering\textcolor{blue}{[인용]}하여 처리를 미룬다는 특징이 있다. 이 경우 개별 데이터의 latency가 길어진다는 문제점이 있다. 특히 가장 처음에 인입되어 대기하는 dataset의 latency가 매우 길어지므로, 스트리밍에서 중요한 tail latency\textcolor{blue}{[인용]}의 손상 정도가 커진다. Throughput-oriented로 인해 발견되는 또 다른 특징으로는 모든 query operation을 GPU로 offloading\textcolor{blue}{[인용]}한다는 것이다. 이는 CPU와 GPU간 데이터 이동으로 인해 발생하는 data transition overhead를 avoid하기 위함이다. Query마다 특정 device만을 이용하는 것은 operator type에 따라 device preference\textcolor{blue}{[인용]}를 반영할 수 없으므로 최적화가 완전히 이루어지지 않는다.
Previous studies introducing GPUs in streaming systems have commonly focused on throughput. They postponed the processing by buffering data to fully utilize the GPUs~\cite{GPU-Online-Stream-Processing}\cite{Gasser}\cite{Toward-GPU-Accelerated-Streaming}.
This causes the latency of individual data to become long.
Since the latency of the early arrived data is very long, the damage of tail latency, which is critical in streaming~\cite{Workload-Aware-Streaming-State-Management}, increases.
Another feature found in the throughput-oriented approaches is that systems planned to offload all query operations to the GPU as much as possible~\cite{GPU-Spark}\cite{GPU-Flink}\cite{Saber}\cite{GPU-Online-Stream-Processing} to avoid data transition overhead caused by data movement between different devices.
However, it is known that distinct device preferences per operator in queries exist~\cite{Fine-Stream}\cite{Performance-Analysis-Of-ETL-Process}. Exploiting a single device separately per query ignores those device preferences and thus misses the chance for further performance optimization.

\vspace{0.1cm}
\noindent{\textbf{Approach using Static Device Preference.}}\label{subsubsec:staticDevicePreference} %최근 FineStream\textcolor{blue}{[인용]}에서 operation level query planning을 진행하였으나, 이 또한 data transition overhead를 무시하기 위해 CPU-GPU integrated chips 위에서 연구를 진행하였다. 그러나 이를 성능이 더 뛰어난 dedicated architecture에 적용하기에는 어렵다. 또한 FineStream의 경우 operator에서 처리하는 데이터의 크기에 따라 달라지는 device preference를 고려하지 않았다. 처리하는 데이터의 크기가 매번 다양하게 변화하는 스트리밍 환경에서는 이와 같은 dynamic device preference를 반영해야 성능이 최적화될 수 있다.
Recently, FineStream~\cite{Fine-Stream} suggested an operation level query planning over the CPU-GPU integrated architecture, which ignores data transition overhead. However, it is hard to apply the proposed idea to a dedicated architecture that has inherent data transmission overhead. In addition, FineStream did not consider device preference that varies depending on the size of data processed by the operator. In streaming environments where the size of processed data changes over time\cite{Q-Flink}, stream processing systems must reflect dynamic device preferences to optimize performance.

%%%%%%%%%%%%%%%%% [Motivation - ourObservations] Figure 1: ourObservations %%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering\includegraphics[width=\linewidth,keepaspectratio]{figures/ourObservations.pdf}
    \vspace{-0.2in}
    \caption{Experiments on dedicated architecture: The bar graph presents normalized execution time, and the line graph shows PCIe overhead ratio.}
    \vspace{-0.2in}
\label{fig:ourObservationsDeprecated}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Our Observations}\label{subsec:ourObservations}

% Dedicated architecture는 integrated architecture 보다 뛰어난 performance를 가진다~\cite{Fine-Stream}. 따라서 throughput과 latency 모두를 최적화해야 하는 스트리밍 워크로드에서는 하드웨어의 성능이 중요하기 때문에 dedicated architecture를 사용할 필요가 있다. 이 section에서는 스트리밍 환경에서 dedicated architecture의 적합성과 고려할 사항들을 밝힌다. 이를 위해 간단한 select-project-filter query의 워크로드를 이용하여 데이터의 크기를 증가시키며 실험하였다.
As mentioned previously, it is generally agreed that dedicated architecture has inherent data transition overhead but better performance than integrated architecture~\cite{Fine-Stream}. %Therefore, in streaming workloads that need to optimize both throughput and latency, it is necessary to use a dedicated architecture with better hardware performance. 
This section motivates the use of operation granularity execution planning over a dedicated architecture despite its overhead, and explains why we need to consider dynamic device preference in \texttt{CG-Spark}'s design. For this, we have conducted an experiment with a simple select-project-filter query as a workload by varying batch data size in the original Spark.

\vspace{0.1cm}
\noindent{\textbf{Low PCIe Overhead for Small Data.}}\label{subsubsec:PCIeOverehadRatio} %Figure~\ref{fig:ourObservations}의 line graph는 data transition overhead의 주요 원인인 PCIe 전송에 소요되는 시간이 전체 수행 시간 중에 차지하는 비율을 나타낸다. PCIe 전송 시간은 GPU profiler인 NVIDIA Nsight Systems를 활용하여 측정하였다. 그래프에서 보여지듯이, 데이터의 크기가 작을 경우 data transition overhead가 매우 작아 무시할 수 있을 정도이다. 이는 비교적 작은 데이터가 인입되는 스트리밍 환경에서는 dedicated architecture에서 발생하는 data transition overhead를 상쇄할 수 있음을 나타낸다. 단, 특정 크기가 넘어갈 경우 오버헤드가 급증하므로 bursty traffic이 들어오는 경우를 고려하여 data transition overhead를 적절히 handling할 필요가 있다.
The line graph in Figure~\ref{fig:ourObservations} shows the ratio of time required for the PCIe transmission to the total execution time, which is the leading factor of data transition overhead. The PCIe transfer time was measured by using a GPU profiler called NVIDIA Nsight Systems. %~\cite{Nvidia-Nsight-Systems}.
As shown in the line graph, it is worthy to note that the PCIe overhead is minimal (i.e., less than 1\%) when the data size is small. This indicates that the data conversion overhead of a dedicated architecture is negligible in streaming environments where relatively small data is continuously ingested. However, after a specific size, the overhead increases dramatically. Therefore, it is also necessary to handle the data conversion overhead appropriately in consideration of bursty traffic.

%%%%%%%%%%%%%%%%% [Design - Overall Systems] Figure 2: overallSystems %%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering\includegraphics[width=\linewidth,keepaspectratio]{figures/overall-systems.png}
    \vspace{-0.2in}
    \caption{\textcolor{blue}{Yellow figures indicate system modules newly implemented in \texttt{CG-Spark}.}}
    \vspace{-0.2in}
\label{fig:overallSystems}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.1cm}
\noindent{\textbf{Necessity of Dynamic Device Preference.}}\label{subsubsec:dynamicDevicePreference} %그림 1에서 막대 그래프는 CPU만을 이용하였을 때, GPU만을 이용하였을때, 그리고 특정 operator만 CPU에 mapping하고 나머지는  모두 GPU에서 실행하였을 때를 비교하여 보여준다. 결과는 CPU만 이용하였을때의 실험 결과를 기준으로 normalizing 하였다. 해당 그래프를 보면 특정 크기를 기준으로 그 값보다 작을 경우 operator들이 CPU를 선호하다가, 그 값을 넘어서면 급격히 GPU를 선호하는 것을 볼 수 있다. 만약 데이터의 크기가 너무 작으면 CPU만 사용하는 것이 가장 좋다. 데이터의 크기가 특정 지점에 도달하면 CPU와 GPU를 섞어서 사용한 경우가 어느 하나의 device만 사용할 때보다 성능이 더 좋음을 알 수 있다. 그러나 데이터 크기가 커지면 CPU 선호도가 급격히 낮아져 모든 operator를 GPU에서 수행하는 것이 적합하다. 더욱 다양한 operator에 대한 실험 내용은 우리의 이전 work~\cite{Performance-Analysis-Of-ETL-Process}에서도 확인할 수 있으며, 이를 통해 dynamic device preference의 필요성이 중요시 됨을 알 수 있다. 특히 data 인입 속도와 주기가 다양하게 변화하는 스트리밍 환경에서는 더욱 필수적이다.
\textcolor{blue}{[TODO: 이전 논문에 썼던 heatmap 가져와서 데이터 크기에 따른 device preference를 확실히 보여주고, 표 같은 것으로 기본 preference를 정리할 것]}
The bar graph in Figure~\ref{fig:ourObservations} also shows the normalized execution times of select-project-filter query when the original Spark is configured with three cases: (1) using only the CPU, (2) using only the GPU, (3) when a specific operator (i.e., filter or project) is mapped to the CPU and all others are executed on the GPU. The execution times were normalized with respect to the run-time when the system is configured with using only the CPU. As shown in the bar graph, if the batch data size is smaller than a certain threshold value (i.e., around 15 KB to 150 KB), some operators prefer the CPU. However, if it exceeds the threshold, the GPU is rapidly preferred. When the data size is too small (i.e., less than 15KB), it is the best choice to use only the CPU. If the data size reaches to a specific size (i.e., 150 KB), the performance is better when the CPU and GPU are mixed rather than using any single device. As the data size increases, CPU affinity drops sharply. Thus, it is appropriate to perform all operators on the GPU. Experiments on more diverse operators can be found in our previous work~\cite{Performance-Analysis-Of-ETL-Process}, which shows that dynamic device preference is essential. In particular, it is more critical in a streaming environment where the data traffic varies continuously.

\vspace{0.1cm}
\noindent{\textbf{Inflection Point.}}\label{subsubsec:inflectionPointNotes} %이와 같이 각 operator를 CPU와 GPU에 다르게 mappping할 때, 성능 분기점이 되는 해당 데이터 크기를 이후 \textit{inflection point}라고 칭한다. 더욱 주목해야 할 부분은 inflection point와 data transition overhead가 급증하기 시작하는 데이터 크기가 동일하다는 것이다. 본 논문에서는 변곡점을 활용하여 데이터 크기에 따른 동적 디바이스 선호도를 지정하는 아이디어를 사용한다.
When mapping each operator differently to the CPU or the GPU, the data size creates a performance branch. %The following documents \textcolor{red}{--- What is the following document? ---}
This papaer refers to this size as \textit{inflection point}. More noteworthy is that the inflection point is the same as the data size where the data transition overhead starts to spike. In this paper, we use the idea of specifying dynamic device preferences according to data size by utilizing inflection points.

% 여기서부터 이전 내용
\begin{comment}
%이전 연구들과 달리, CG-Spark에서는 query 내의 개별적인 operator를 discrete CPU와 GPU에 다르게 mapping하는 operator granularity query planning을 사용한다. 이 때 가장 관건이 되는 사항은 한번에 처리하려는 데이터의 크기와 각 operator의 device preference이다. 우리는 데이터 크기에 따라 device preference가 달라진다는 것을 보이기 위해 실험을 진행하였다. 워크로드는 간단한 select-project-filter query를 이용하였고 데이터의 크기를 증가시키며 실험하였다. 그림 1에서 막대 그래프는 CPU만을 이용하였을 때, GPU만을 이용하였을때, 그리고 특정 operator만 CPU에 mapping하고 나머지는  모두 GPU에서 실행하였을 때를 비교하여 보여준다. 결과는 CPU만 이용하였을때의 실험 결과를 기준으로 normalizing 하였다. 해당 그래프를 보면 특정 크기를 기준으로 그 값보다 작을 경우 operator들이 CPU를 선호하다가, 그 값을 넘어서면 급격히 GPU를 선호하는 것을 볼 수 있다. 만약 데이터의 크기가 너무 작으면 CPU만 사용하는 것이 가장 좋다. 데이터의 크기가 특정 지점에 도달하면 CPU와 GPU를 섞어서 사용한 경우가 어느 하나의 device만 사용할 때보다 성능이 더 좋음을 알 수 있다. 그러나 데이터 크기가 커지면 CPU 선호도가 급격히 낮아져 모든 operator를 GPU에서 수행하는 것이 적합하다. 더욱 다양한 operator에 대한 실험 내용은 우리의 이전 work~\cite{Performance-Analysis-Of-ETL-Process}에서도 확인할 수 있으며, 이를 통해 dynamic device preference의 필요성이 중요시 됨을 알 수 있다. 한편, 이와 같이 각 operator를 CPU와 GPU에 다르게 mappping할 때, 성능 분기점이 되는 해당 데이터 크기를 이후 \textit{inflection point}라고 칭한다.
Unlike previous studies, \texttt{CG-Spark} uses an operator granularity planning that maps individual operator within a query to dedicated CPUs and GPUs dynamically. The most important issue is the size of data in a single process cycle and the device preference of each operator.

To explain this further,
%Further experiment shows that device preference varies according to data size. 
we have conducted an experiment with a simple select-project-filter query as a workload by increasing the size of the data.
%used a simple select-project-filter query as a workload and experimented with increasing the size of the data. 
%The bar graph in 
Figure~\ref{fig:ourObservations} shows the normalized execution times of four different settings where the original Spark is configured with the cases using only the CPU, using only the GPU, when a specific operator is mapped to the CPU and all others are executed on the GPU. The performance results were normalized based on the run-time when the system is configured with using only the CPU. As shown in Figure~\ref{fig:ourObservations}, if the size is smaller than a specific value, some operators prefer the CPU, and if it exceeds the one, the GPU is rapidly preferred. When the data size is too small, it is the best choice to use only the CPU. If the data size reaches a specific point, the performance is better when the CPU and GPU are mixed rather than using any single device. As the data size increases, CPU affinity drops sharply, so it is appropriate to perform all operators on the GPU. Experiments on more diverse operators can be found in the previous work~\cite{Performance-Analysis-Of-ETL-Process}, which shows that dynamic device preference is essential. Meanwhile, when mapping each operator differently to the CPU and GPU, the data size creates a performance branch. The following documents refer to this size as \textit{inflection point}.

%위 실험의 근거를 얻기 위해 data transition overhead를 분석하는 추가적인 실험을 진행하였다. 워크로드는 이전과 동일하게 설정하였으며, GPU profiler인 NVIDIA Nsight Systems를 활용하여 data transition overhead의 주요 원인인 PCIe 전송에 소요되는 시간이 전체 수행 시간 중에 차지하는 비율을 계산하였다. 그림 1의 line graph에서 그 결과를 확인할 수 있다. 요약하면 데이터의 크기가 작을 경우 data transition overhead가 매우 작아 무시할 수 있을 정도이지만, 특정 크기가 넘어갈 경우 오버헤드가 급증한다. 더욱 주목해야 할 부분은 bar graph의 inflection point와 data transition overhead가 급증하기 시작하는 데이터 크기가 동일하다는 것이다.
To obtain the basis for the above experiment, we conducted additional experiments to analyze the data transition overhead. The workload is the same as before. We calculated the ratio of the time required for PCIe transmission to the total execution time, which is the main factor of data transition overhead. For experiment, we used NVIDIA Nsight Systems, a GPU profiler. The results are shown in the line graph in Figure~\ref{fig:ourObservations}. In short, if the data size is small, the data transition overhead is too small to be ignored. However, if the data size exceeds a certain point, the overhead increases dramatically. More noteworthy is that the inflection point of the bar graph and the data size at which the data transition overhead starts to increase rapidly are the same.

%위와 같은 결과들을 기준으로, 본 논문에서는 infection point와 현재 데이터 크기를 비교하여 operator를 device에 dynamic하게 mapping하고, 이를 통해 전체적인 throughput 향상을 도모한다. 또한 데이터 크기가 작을 경우 알맞은 device mapping을 통해 데이터가 곧바로 처리될 수 있도록 한다. 따라서 GPU 활용을 위해 실시간 데이터를 buffering하여 latency가 손상되는 것을 막는다. 이를 위해 \texttt{CG-Spark}는 user-specified deadline을 고려하여 적절한 크기의 micro-batch를 생성하고, 그에 따라 operator마다 dynamic하게 device를 mapping한다. 이 때 시스템 안정성을 위해 GPU의 free memory capcaity를 반영한 rule을 추가적으로 사용한다. 자세한 설계는 Chapter~\ref{sec:design}에서 설명한다.
Reflecting on our observations, \texttt{CG-Spark} dynamically map operators to devices based on current data sizes to improve overall throughput. In addition, even though the data size is small, \texttt{CG-Spark} process data immediately through appropriate device mapping. Thus, our systems prevent severe latency generated by buffering real-time data for GPU utilization. For our system goals, \texttt{CG-Spark} creates a micro-batch of an appropriate size in consideration of the user-specified deadline. Then it dynamically maps devices for each operator according to the data size in the micro-batch. During a device mapping process, \texttt{CG-Spark} uses an additional rule aware of available GPU memory capacity to prevent out-of-memory failure. Detailed design is explained in Chapter~\ref{sec:design}.

%둘째로 operator type에 따라 device preference가 확연히 다르다. 이는 이전 연구들에서도 밝혀진 바 있다\textcolor{blue}{[인용]}. 이전 연구의 내용과 그림 1에서 진행한 실험을 바탕으로, 기본적인 device preference를 table1과 같이 정리하였다. 그러나 이러한 preference는 처리하려는 데이터 크기에 따라 dynamic하게 바뀐다. 그림 1의 결과에서와 같이, 데이터의 크기가 inflection point 이상으로 커지면 무조건 GPU에서 실행하는 것이 성능상의 이득임을 알 수 있다. 즉 inflection point는 operation granularity query planning 수행 시 가장 중요한 기준점이 된다. CG-Spark에서는 이를 이용한 cost model과 device mapping rule을 지정하여 stream processing에서 tail latency를 최소화하고 average throughput을 최적화한다.
%Second, device preference differs significantly according to operator type. This has also been shown in previous studies~\cite{Fine-Stream}\cite{Performance-Analysis-Of-ETL-Process}. Based on the contents of the previous study and the experiment results in Figure~\ref{fig:ourObservations}, basic device preferences are summarized as follows.
%\begin{itemize}
    %\item CPU preference: Aggregation, Filtering, Exchange
    %\item Neutral: Projection, Join
    %\item GPU preference: Scan, Sorting
%\end{itemize}
%However, these preferences change dynamically according to the size of the data to be processed. As shown in the result of Figure~\ref{fig:ourObservations}, when the size of the data becomes larger than the inflection point, it is better in terms of performance to run on the GPU unconditionally. That is, the inflection point becomes the most important reference point when performing operation granularity query planning. \texttt{CG-Spark} minimizes tail latency in stream processing and optimizes average throughput by specifying a cost model and device mapping rule using the inflection point concept.
\end{comment}
